Differentially Private Model Compression

Recent papers have shown that large pre-trained language models (LLMs) such as BERT, GPT-2 can be fine-tuned on private data to achieve performance comparable to non-private models for many downstream Natural Language Processing (NLP) tasks while simultaneously guaranteeing differential privacy. The inference cost of these models -- which consist of hundreds of millions of parameters -- however, can be prohibitively large. Hence, often in practice, LLMs are compressed before they are deployed in specific applications. In this paper, we initiate the study of differentially private model compression and propose frameworks for achieving 50% sparsity levels while maintaining nearly full performance. We demonstrate these ideas on standard GLUE benchmarks using BERT models, setting benchmarks for future research on this topic.

==> body/ExperimentalSetUp.tex <==
\section{Experimental Set Up}



Our main goal in all of the experiments is to produce compressed models that achieve sparsity levels that $50\%$ of their original, full-size counterpart.
%
Throughout the paper, we refer to the full-size pre-trained models, all of which are BERT~\footnote{We use Huggingface's \texttt{bert-base-uncased}.} in the experiments, as teacher models, and the compressed models (half of BERT, i.e. 6 out of the 12 layers) as student models. 
%
One of the assumptions made here is that model sparsity can be used as a proxy for measuring computational cost at inference time. 
%
Below we see details of the experimental setup.
%
We include software specifications in Appendix~\ref{app:spec}.



\paragraph{Tasks and datasets.}
We experiment with the following set of $4$ tasks from the GLUE benchmark~\cite{glue}: MNLI (Multi-Genre Natural Language Inference Corpus), QQP (Quora Question Pairs), QNLI (Stanford Question Answering Dataset) and SST-2 (Stanford Sentiment Treebank). These are all classification tasks covering natural language inference, question answering, paraphrasing and sentiment analysis, with $3$, $2$, $2$ and $2$ target classes and $393k$, $364k$, $105k$ and $67k$ training samples respectively.


\paragraph{Model initialization.}
We initialize the student model in three different ways: (1) Random, (2) Zero-shot (PT), where we use the weights from  6 of pre-trained BERT's layers to initialize the student  and (3) Pre-trained, where we use Huggingface's pre-trained compressed BERT model, DistilBERT. The difference between these models is how well they transfer knowledge, as the random initializaiton has basically no information to transfer, the zero-shot might have some information and the pre-trained one would be the best initialization, as the student model with its compressed architecture has directly been trained. 


\paragraph{Training and privacy parameters.} In all our experiments, we have set the target privacy budget to be $\epsilon=4.0$, with $\delta=\frac{1}{10N}$ where $N$ is the number of samples in the given dataset. We provide hyper-parameter details for all the experiments in the Appendix. 
%









==> tables/better_teacher.tex <==
\begin{tabular}{c | c | c | c | c c c c}
\hline 
Model & Initialization & Teacher & Training & MNLI & QQP & QNLI & SST-2 \\
\hline 
$\textnormal{BERT}_{\textsc{BASE}}$ & - & - & Finetune & 77.8 & 84.7 & 87.8 & TBD \\
\hline
Student & Zero-shot (PT) & $\textnormal{BERT}_{\textsc{BASE}}$ & Distillation & 72.8 & 82.6 & 83.0 & TBD  \\
Student & Zero-shot (PT) & $\textnormal{BERT}_{\textsc{LARGE}}$ & Distillation & 72.4 & 81.1 & 83.1 & TBD \\
Student & Zero-shot (PT) & $\textnormal{BERT}_{\textsc{BASE}}$ without DP & Distillation & TBD & TBD & TBD & TBD \\
\hline
\end{tabular}

==> tables/rand-zeroshot-pretrained.tex <==
\begin{tabular}{c | c | c | c | c c c c}
\hline 
Model & Initialization & Teacher & Training & MNLI & QQP & QNLI & SST-2 \\
\hline 
$\textnormal{BERT}_{\textsc{BASE}}$ & - & - & Finetune & 77.8 & 84.7 & 87.8 & TBD \\
\hline
Student & Random & - & Finetune & 55.1 & 74.0 & 59.4 & TBD \\
Student & Random & $\textnormal{BERT}_{\textsc{BASE}}$ & Distillation & TBD & 73.1 & 59.2 & TBD \\
\hline 
Student & Zero-shot (PT) & - & Finetune & 71.7 & 82.4 & 83.2 & TBD \\
Student & Zero-shot (PT) & $\textnormal{BERT}_{\textsc{BASE}}$ & Distillation & 72.8 & 82.6 &  83.0 & TBD \\
\hline
Student & Zero-shot (FT) & - & Finetune & 71.3 & 81.8 & 83.4 & TBD \\
Student & Zero-shot (FT) & $\textnormal{BERT}_{\textsc{BASE}}$ & Distillation & 72.3 & 82.1 & 82.9 & TBD \\
\hline
Student & Pre-trained & - & Finetune & 73 & 84.3 & 82.8 & TBD \\
Student & Pre-trained & $\textnormal{BERT}_{\textsc{BASE}}$ & Distillation & 72.9 & 83.7 & 83.0 & TBD \\
\hline
\end{tabular}

